The Deterministic Part of IPC-4: An Overview

We provide an overview of the organization and results of the deterministic part of the 4th International Planning Competition, i.e., of the part concerned with evaluating systems doing deterministic planning. IPC-4 attracted even more competing systems than its already large predecessors, and the competition event was revised in several important respects. After giving an introduction to the IPC, we briefly explain the main differences between the deterministic part of IPC-4 and its predecessors. We then introduce formally the language used, called PDDL2.2 that extends PDDL2.1 by derived predicates and timed initial literals. We list the competing systems and overview the results of the competition. The entire set of data is far too large to be presented in full. We provide a detailed summary; the complete data is available in an online appendix. We explain how we awarded the competition prizes.

==> RESULTS/gnus <==
cd AIRPORT/NONTEMPORAL/GNUPLOT ; gnuplot <  MAKESPAN.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd AIRPORT/NONTEMPORAL/GNUPLOT ; gnuplot <  NRACTIONS.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd AIRPORT/NONTEMPORAL/GNUPLOT ; gnuplot <  TIME_OPTIMAL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd AIRPORT/NONTEMPORAL/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL_1.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd AIRPORT/NONTEMPORAL/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL_2.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd AIRPORT/NONTEMPORAL/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL_ALL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd AIRPORT/TEMPORAL/GNUPLOT ; gnuplot <  MAKESPAN.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd AIRPORT/TEMPORAL/GNUPLOT ; gnuplot <  NRACTIONS.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd AIRPORT/TEMPORAL/GNUPLOT ; gnuplot <  TIME_OPTIMAL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd AIRPORT/TEMPORAL/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd AIRPORT/TEMPORAL_TIMEWINDOWS/GNUPLOT ; gnuplot <  MAKESPAN.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd AIRPORT/TEMPORAL_TIMEWINDOWS/GNUPLOT ; gnuplot <  NRACTIONS.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd AIRPORT/TEMPORAL_TIMEWINDOWS/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd AIRPORT/TEMPORAL_TIMEWINDOWS_COMPILED/GNUPLOT ; gnuplot <  MAKESPAN.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd AIRPORT/TEMPORAL_TIMEWINDOWS_COMPILED/GNUPLOT ; gnuplot <  NRACTIONS.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd AIRPORT/TEMPORAL_TIMEWINDOWS_COMPILED/GNUPLOT ; gnuplot <  TIME_OPTIMAL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd AIRPORT/TEMPORAL_TIMEWINDOWS_COMPILED/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PIPESWORLD/NOTANKAGE_NONTEMPORAL/GNUPLOT ; gnuplot <  MAKESPAN.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PIPESWORLD/NOTANKAGE_NONTEMPORAL/GNUPLOT ; gnuplot <  NRACTIONS.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PIPESWORLD/NOTANKAGE_NONTEMPORAL/GNUPLOT ; gnuplot <  TIME_OPTIMAL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PIPESWORLD/NOTANKAGE_NONTEMPORAL/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL_1.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PIPESWORLD/NOTANKAGE_NONTEMPORAL/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL_2.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PIPESWORLD/NOTANKAGE_NONTEMPORAL/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL_ALL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PIPESWORLD/NOTANKAGE_TEMPORAL/GNUPLOT ; gnuplot <  MAKESPAN.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PIPESWORLD/NOTANKAGE_TEMPORAL/GNUPLOT ; gnuplot <  NRACTIONS.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PIPESWORLD/NOTANKAGE_TEMPORAL/GNUPLOT ; gnuplot <  TIME_OPTIMAL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PIPESWORLD/NOTANKAGE_TEMPORAL/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PIPESWORLD/NOTANKAGE_TEMPORAL_DEADLINES/GNUPLOT ; gnuplot <  MAKESPAN.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PIPESWORLD/NOTANKAGE_TEMPORAL_DEADLINES/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PIPESWORLD/NOTANKAGE_TEMPORAL_DEADLINES_CO/GNUPLOT ; gnuplot <  TIME_OPTIMAL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PIPESWORLD/NOTANKAGE_TEMPORAL_DEADLINES_CO/GNUPLOT ; gnuplot <  MAKESPAN.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PIPESWORLD/TANKAGE_NONTEMPORAL/GNUPLOT ; gnuplot <  MAKESPAN.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PIPESWORLD/TANKAGE_NONTEMPORAL/GNUPLOT ; gnuplot <  NRACTIONS.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PIPESWORLD/TANKAGE_NONTEMPORAL/GNUPLOT ; gnuplot <  TIME_OPTIMAL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PIPESWORLD/TANKAGE_NONTEMPORAL/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL_1.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PIPESWORLD/TANKAGE_NONTEMPORAL/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL_2.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PIPESWORLD/TANKAGE_NONTEMPORAL/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL_ALL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PIPESWORLD/TANKAGE_TEMPORAL/GNUPLOT ; gnuplot <  MAKESPAN.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PIPESWORLD/TANKAGE_TEMPORAL/GNUPLOT ; gnuplot <  NRACTIONS.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PIPESWORLD/TANKAGE_TEMPORAL/GNUPLOT ; gnuplot <  TIME_OPTIMAL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PIPESWORLD/TANKAGE_TEMPORAL/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PROMELA/OPTICAL_TELEGRAPH/GNUPLOT ; gnuplot <  MAKESPAN.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PROMELA/OPTICAL_TELEGRAPH/GNUPLOT ; gnuplot <  NRACTIONS.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PROMELA/OPTICAL_TELEGRAPH/GNUPLOT ; gnuplot <  TIME_OPTIMAL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PROMELA/OPTICAL_TELEGRAPH/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL_ALL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PROMELA/OPTICAL_TELEGRAPH_DERIVEDPREDIC/GNUPLOT ; gnuplot <  MAKESPAN.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PROMELA/OPTICAL_TELEGRAPH_DERIVEDPREDIC/GNUPLOT ; gnuplot <  NRACTIONS.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PROMELA/OPTICAL_TELEGRAPH_DERIVEDPREDIC/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL_ALL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PROMELA/OPTICAL_TELEGRAPH_FLUENTS/GNUPLOT ; gnuplot <  NRACTIONS.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PROMELA/OPTICAL_TELEGRAPH_FLUENTS/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL_ALL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PROMELA/PHILOSOPHERS/GNUPLOT ; gnuplot <  MAKESPAN.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PROMELA/PHILOSOPHERS/GNUPLOT ; gnuplot <  NRACTIONS.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PROMELA/PHILOSOPHERS/GNUPLOT ; gnuplot <  TIME_OPTIMAL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PROMELA/PHILOSOPHERS/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL_ALL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PROMELA/PHILOSOPHERS_DERIVEDPREDICATES/GNUPLOT ; gnuplot <  MAKESPAN.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PROMELA/PHILOSOPHERS_DERIVEDPREDICATES/GNUPLOT ; gnuplot <  NRACTIONS.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PROMELA/PHILOSOPHERS_DERIVEDPREDICATES/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL_ALL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PROMELA/PHILOSOPHERS_FLUENTS/GNUPLOT ; gnuplot <  MAKESPAN.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PROMELA/PHILOSOPHERS_FLUENTS/GNUPLOT ; gnuplot <  NRACTIONS.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PROMELA/PHILOSOPHERS_FLUENTS/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL_ALL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PSR/LARGE/GNUPLOT ; gnuplot <  MAKESPAN.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PSR/LARGE/GNUPLOT ; gnuplot <  NRACTIONS.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PSR/LARGE/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL_ALL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PSR/MIDDLE/GNUPLOT ; gnuplot <  MAKESPAN.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PSR/MIDDLE/GNUPLOT ; gnuplot <  NRACTIONS.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PSR/MIDDLE/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL_ALL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PSR/MIDDLE_COMPILED/GNUPLOT ; gnuplot <  NRACTIONS.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PSR/MIDDLE_COMPILED/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL_ALL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PSR/SMALL/GNUPLOT ; gnuplot <  MAKESPAN.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PSR/SMALL/GNUPLOT ; gnuplot <  NRACTIONS.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PSR/SMALL/GNUPLOT ; gnuplot <  TIME_OPTIMAL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PSR/SMALL/GNUPLOT ; gnuplot <  TIME_OPTIMAL_1.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PSR/SMALL/GNUPLOT ; gnuplot <  TIME_OPTIMAL_2.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PSR/SMALL/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL_1.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PSR/SMALL/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL_2.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd PSR/SMALL/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL_ALL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd SATELLITE/COMPLEX/GNUPLOT ; gnuplot <  MAKESPAN.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd SATELLITE/COMPLEX/GNUPLOT ; gnuplot <  NRACTIONS.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd SATELLITE/COMPLEX/GNUPLOT ; gnuplot <  TIME_OPTIMAL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd SATELLITE/COMPLEX/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd SATELLITE/COMPLEX_TIMEWINDOWS/GNUPLOT ; gnuplot <  MAKESPAN.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd SATELLITE/COMPLEX_TIMEWINDOWS/GNUPLOT ; gnuplot <  METRICVALUE.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd SATELLITE/COMPLEX_TIMEWINDOWS/GNUPLOT ; gnuplot <  NRACTIONS.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd SATELLITE/COMPLEX_TIMEWINDOWS/GNUPLOT ; gnuplot <  TIME_ALL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd SATELLITE/COMPLEX_TIMEWINDOWS_COMPILED/GNUPLOT ; gnuplot <  NRACTIONS.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd SATELLITE/COMPLEX_TIMEWINDOWS_COMPILED/GNUPLOT ; gnuplot <  TIME_ALL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd SATELLITE/NUMERIC/GNUPLOT ; gnuplot <  METRICVALUE.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd SATELLITE/NUMERIC/GNUPLOT ; gnuplot <  NRACTIONS.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd SATELLITE/NUMERIC/GNUPLOT ; gnuplot <  TIME_ALL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd SATELLITE/STRIPS/GNUPLOT ; gnuplot <  MAKESPAN.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd SATELLITE/STRIPS/GNUPLOT ; gnuplot <  NRACTIONS.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd SATELLITE/STRIPS/GNUPLOT ; gnuplot <  TIME_OPTIMAL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd SATELLITE/STRIPS/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL_ALL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd SATELLITE/TIME/GNUPLOT ; gnuplot <  MAKESPAN.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd SATELLITE/TIME/GNUPLOT ; gnuplot <  NRACTIONS.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd SATELLITE/TIME/GNUPLOT ; gnuplot <  TIME_OPTIMAL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd SATELLITE/TIME/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd SATELLITE/TIME_TIMEWINDOWS/GNUPLOT ; gnuplot <  MAKESPAN.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd SATELLITE/TIME_TIMEWINDOWS/GNUPLOT ; gnuplot <  NRACTIONS.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd SATELLITE/TIME_TIMEWINDOWS/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd SATELLITE/TIME_TIMEWINDOWS_COMPILED/GNUPLOT ; gnuplot <  MAKESPAN.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd SATELLITE/TIME_TIMEWINDOWS_COMPILED/GNUPLOT ; gnuplot <  NRACTIONS.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd SATELLITE/TIME_TIMEWINDOWS_COMPILED/GNUPLOT ; gnuplot <  TIME_ALL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd SETTLERS/IPC_3/GNUPLOT ; gnuplot <  METRICVALUE.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd SETTLERS/IPC_3/GNUPLOT ; gnuplot <  NRACTIONS.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd SETTLERS/IPC_3/GNUPLOT ; gnuplot <  TIME_ALL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd UMTS/FLAW_TEMPORAL/GNUPLOT ; gnuplot <  MAKESPAN.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd UMTS/FLAW_TEMPORAL/GNUPLOT ; gnuplot <  NRACTIONS.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd UMTS/FLAW_TEMPORAL/GNUPLOT ; gnuplot <  TIME_OPTIMAL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd UMTS/FLAW_TEMPORAL/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd UMTS/FLAW_TEMPORAL_TIMEWINDOWS/GNUPLOT ; gnuplot <  MAKESPAN.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd UMTS/FLAW_TEMPORAL_TIMEWINDOWS/GNUPLOT ; gnuplot <  NRACTIONS.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd UMTS/FLAW_TEMPORAL_TIMEWINDOWS/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd UMTS/FLAW_TEMPORAL_TIMEWINDOWS_COMPI/GNUPLOT ; gnuplot <  NRACTIONS.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd UMTS/FLAW_TEMPORAL_TIMEWINDOWS_COMPI/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd UMTS/TEMPORAL/GNUPLOT ; gnuplot <  MAKESPAN.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd UMTS/TEMPORAL/GNUPLOT ; gnuplot <  NRACTIONS.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd UMTS/TEMPORAL/GNUPLOT ; gnuplot <  TIME_OPTIMAL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd UMTS/TEMPORAL/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd UMTS/TEMPORAL_TIMEWINDOWS/GNUPLOT ; gnuplot <  MAKESPAN.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd UMTS/TEMPORAL_TIMEWINDOWS/GNUPLOT ; gnuplot <  NRACTIONS.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd UMTS/TEMPORAL_TIMEWINDOWS/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd UMTS/TEMPORAL_TIMEWINDOWS_COMPILED/GNUPLOT ; gnuplot <  NRACTIONS.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS
cd UMTS/TEMPORAL_TIMEWINDOWS_COMPILED/GNUPLOT ; gnuplot <  TIME_SUBOPTIMAL.GNU; cd /cygdrive/c/Dokumente\ und\ Einstellungen/edelkamp/Desktop/Closer/RESULTS

